Quantifying and qualifying trust: Spectral decomposition of trust networks

In a previous FAST paper, I presented a quantitative model of the process of trust building, and showed that trust is accumulated like wealth: the rich get richer. This explained the pervasive phenomenon of adverse selection of trust certificates, as well as the fragility of trust networks in general. But a simple explanation does not always suggest a simple solution. It turns out that it is impossible to alter the fragile distribution of trust without sacrificing some of its fundamental functions. A solution for the vulnerability of trust must thus be sought elsewhere, without tampering with its distribution. This observation was the starting point of the present paper. It explores a different method for securing trust: not by redistributing it, but by mining for its sources. The method used to break privacy is thus also used to secure trust. A high level view of the mining methods that connect the two is provided in terms of *similarity networks*, and *spectral decomposition* of similarity preserving maps. This view may be of independent interest, as it uncovers a common conceptual and structural foundation of mathematical classification theory on one hand, and of the spectral methods of graph clustering and data mining on the other hand.

==> AA-PICS/spectral.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Sep 13 18:40:59 PDT 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="90" y-min="2.5" y-max="52.5" auto-bounding="true">
%<multicurve stroke-width= "0.5"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(20,40);(20,40);(80,40);(80,40)"
%	 />
%<multicurve stroke-width= "0.2"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "double-head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(85,35);(85,35);(75,10);(75,10)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,40)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\alice$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,40)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\bob$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,42.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgOneBack$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(82.5,52.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(77,5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\intoOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,2.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\intoOneBack$
%</text>
%<multicurve stroke-width= "0.5"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(30,5);(30,5);(70,5);(70,5)"
%	 />
%<multicurve stroke-width= "0.5"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 left-arrow= "reverse-head"
%	 points= "(80,10);(80,10);(90,35);(90,35)"
%	 />
%<multicurve stroke-width= "0.5"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "double-head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(10,35);(10,35);(20,10);(20,10)"
%	 />
%<multicurve stroke-width= "0.2"
%	 arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 left-arrow= "reverse-head"
%	 points= "(25,10);(25,10);(15,35);(15,35)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(87,23)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\rightout$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(79,23)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\rightin$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(22,22)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\leftin$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13,23)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\leftout$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(90,52.5)
\psline[linewidth=0.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(20,40)(80,40)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->>}(85,35)(75,10)
\rput(10,40){$\alice$}
\rput(90,40){$\bob$}
\rput(50,42.5){$\msgOne$}
\rput(24,5){$\msgOneBack$}
\rput[b](82.5,52.5){}
\rput(77,5){$\intoOne$}
\rput(50,2.5){$\intoOneBack$}
\psline[linewidth=0.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(30,5)(70,5)
\psline[linewidth=0.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{>->}(80,10)(90,35)
\psline[linewidth=0.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->>}(10,35)(20,10)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{>->}(25,10)(15,35)
\rput[l](87,23){$\rightout$}
\rput[r](79,23){$\rightin$}
\rput[l](22,22){$\leftin$}
\rput[r](13,23){$\leftout$}
\end{pspicture}

